SIPDO: Closed-Loop Prompt Optimization via Synthetic Data Feedback

Prompt quality plays a critical role in the performance of large language models (LLMs), motivating a growing body of work on prompt optimization. Most existing methods optimize prompts over a fixed dataset, assuming static input distributions and offering limited support for iterative improvement. We introduce SIPDO (Self-Improving Prompts through Data-Augmented Optimization), a closed-loop framework for prompt learning that integrates synthetic data generation into the optimization process. SIPDO couples a synthetic data generator with a prompt optimizer, where the generator produces new examples that reveal current prompt weaknesses and the optimizer incrementally refines the prompt in response. This feedback-driven loop enables systematic improvement of prompt performance without assuming access to external supervision or new tasks. Experiments across question answering and reasoning benchmarks show that SIPDO outperforms standard prompt tuning methods, highlighting the value of integrating data synthesis into prompt learning workflows.

==> sections/6-limitation.tex <==
\section*{Limitations and Discussions}
Although SIPDO yields clear improvements on standard reasoning benchmarks, it has two main limitations. First, all experiments were run
on clean public datasets; we have not yet tested
SIPDO on messier, domain-specific collections
such as financial filings or clinical notes, where
labeling rules and text quality vary widely. Second, an adaptive, automated system in which each stage generates its own prompts for both the Data Generator and the Auto-Prompt Optimizer could produce a fully automated prompt-generation module that—using model feedback—proposes, tests, and refines its prompts at each stage. By closing the loop on prompt creation, SIPDO could adapt to new domains and data types without manual tuning, making it more scalable and broadly applicable.


